New Convex Programs for Fisher's Market Model and its Generalizations

We present the following results pertaining to Fisher's market model: -We give two natural generalizations of Fisher's market model: In model M_1, sellers can declare an upper bound on the money they wish to earn (and take back their unsold good), and in model M_2, buyers can declare an upper bound on the amount to utility they wish to derive (and take back the unused part of their money). -We derive convex programs for the linear case of these two models by generalizing a convex program due to Shmyrev and the Eisenberg-Gale program, respectively. -We generalize the Arrow-Hurwicz theorem to the linear case of these two models, hence deriving alternate convex programs. -For the special class of convex programs having convex objective functions and linear constraints, we derive a simple set of rules for constructing the dual program (as simple as obtaining the dual of an LP). Using these rules we show a formal relationship between the two seemingly different convex programs for linear Fisher markets, due to Eisenberg-Gale and Shmyrev; the duals of these are the same, upto a change of variables.

==> macros.tex <==
 \newenvironment{proof}{\noindent {\bf Proof:}}{$\Box$ \medskip}
% \newenvironment{proofoffact}{\noindent {\sc Proof of Fact:}}{$\Box$ \medskip}
% \newenvironment{proofofclaim}{\noindent {\sc Proof of Claim:}}{$\Box$ \medskip}
% \newenvironment{proofoflemma}{\noindent {\sc Proof of Lemma:}}{$\Box$ \medskip}

%%Version Feb 3 2001; last edited by SA
% Feb 13, 2001: LT adds following macros:
%  \logred, \conl, \genclass, \cogenclass, \size,
%  \floor, \ceil, \comp, \ffigure, \ffigureh
%  \iff, \implies, \sigmatwo, \sigmathree, \pitwo,
%  \scand, \scor, \scnot, \scyes
%Feb20 SA added \sig and \pip for boldface polynomial hierarchy
%% Macros for complexity theory notation
%% Complexity classes
\renewcommand\P{\mbox{\bf P}\xspace}
\newcommand\NP{\mbox{\bf NP}\xspace}
\newcommand\cnp{\mbox{\bf coNP}\xspace}
\newcommand\sigmatwo{\mbox{\bf $\Sigma_2$}\xspace}
\newcommand\sigmathree{\mbox{\bf $\Sigma_3$}\xspace}
\newcommand\pitwo{\mbox{\bf $\Pi_2$}\xspace}
\newcommand\rp{\mbox{\bf RP}\xspace}
\newcommand\zpp{\mbox{\bf ZPP}\xspace}
\newcommand\bpp{\mbox{\bf BPP}\xspace}
\newcommand\ph{\mbox{\bf PH}\xspace}
\newcommand\pspace{\mbox{\bf PSPACE}\xspace}
\newcommand\npspace{\mbox{\bf NPSPACE}\xspace}
\newcommand\dl{\mbox{\bf L}\xspace}

\newcommand\conl{\mbox{\bf coNL}\xspace}
\newcommand\sharpp{\mbox{\#{\bf P}}\xspace}
\newcommand\parityp{\mbox{$\oplus$ {\bf P}}\xspace}
\newcommand\ip{\mbox{\bf IP}\xspace}
\newcommand\pcp{\mbox{\bf PCP}}
\newcommand\dtime{\mbox{\bf DTIME}}
\newcommand\ntime{\mbox{\bf NTIME}}
\newcommand\dspace{\mbox{\bf SPACE}\xspace}
\newcommand\nspace{\mbox{\bf NSPACE}\xspace}
\newcommand\cnspace{\mbox{\bf coNSPACE}\xspace}
\newcommand\exptime{\mbox{\bf EXPTIME}\xspace}
\newcommand\nexptime{\mbox{\bf NEXPTIME}\xspace}
\newcommand\genclass{\mbox{$\cal C$}\xspace}
\newcommand\cogenclass{\mbox{\bf co$\cal C$}\xspace}
\newcommand\size{\mbox{\bf SIZE}\xspace}
\newcommand\sig{\mathbf \Sigma}
\newcommand\pip{\mathbf \Pi}

%%Computational problems

\newcommand\sat{\mbox{SAT}\xspace}
\newcommand\tsat{\mbox{3SAT}\xspace}
\newcommand\maxtsat{\mbox{MAX3SAT}\xspace}
\newcommand\tqbf{\mbox{TQBF}\xspace}


%% Notation for integers, natural numbers, reals, fractions, sets, cardinalities
%%and so on

\newcommand\bz{\mbox{\bf Z}}
\newcommand\nat{\mbox{\bf N}}
\newcommand\rea{\mbox{\bf R}}
\newcommand\B{\{0,1\}}      % boolean alphabet  use in math mode
\newcommand\Bs{\{0,1\}^*}   % B star            use in math mode
\newcommand\true{\mbox{\sc True}}
\newcommand\false{\mbox{\sc False}}
\DeclareRobustCommand{\fracp}[2]{{#1 \overwithdelims()#2}}
\DeclareRobustCommand{\fracb}[2]{{#1 \overwithdelims[]#2}}
\newcommand{\marginlabel}[1]%
{\mbox{}\marginpar{\it{\raggedleft\hspace{0pt}#1}}}
\newcommand\card[1]{\left| #1 \right|} %cardinality of set S; usage \card{S}
\newcommand\set[1]{\left\{#1\right\}} %usage \set{1,2,3,,}
%\newcommand\poly{\mbox{poly}}  %usage \poly(n)
\newcommand{\floor}[1]{\lfloor\, $#1$\,\rfloor}
\newcommand{\ceil}[1]{\lceil\, $#1$\,\rceil}
\newcommand{\comp}[1]{\overline{#1}}


%% Various things to write in small caps

\def\scand{\mbox{\sc and}}
\def\scor{\mbox{\sc or}}
\def\scnot{\mbox{\sc not}}
\def\scyes{\mbox{\sc yes}}


%% short-hands for relational simbols

%\newcommand\to{\rightarrow}
\newcommand{\from}{:}
\newcommand\xor{\oplus}
\newcommand\bigxor{\bigoplus}
\newcommand{\logred}{\leq_{\log}}
\def\iff{\Leftrightarrow}
\def\implies{\Rightarrow}


%% probability stuff
\newcommand\prob{\mbox{\bf Pr}}
\newcommand\E{\mbox{\bf E}}
\newcommand\var{\mbox{\bf Var}}



%% macros to write pseudo-code

\newlength{\pgmtab}  %  \pgmtab is the width of each tab in the
\setlength{\pgmtab}{1em}  %  program environment
 \newenvironment{program}{\renewcommand{\baselinestretch}{1}%
\begin{tabbing}\hspace{0em}\=\hspace{0em}\=%
\hspace{\pgmtab}\=\hspace{\pgmtab}\=\hspace{\pgmtab}\=\hspace{\pgmtab}\=%
\hspace{\pgmtab}\=\hspace{\pgmtab}\=\hspace{\pgmtab}\=\hspace{\pgmtab}\=%
\+\+\kill}{\end{tabbing}\renewcommand{\baselinestretch}{\intl}}
% \newcommand {\BEGIN}{{\bf begin\ }}
% \newcommand {\ELSE}{{\bf else\ }}
% \newcommand {\IF}{{\bf if\ }}
% \newcommand {\FOR}{{\bf for\ }}
% \newcommand {\TO}{{\bf to\ }}
% \newcommand {\DO}{{\bf do\ }}
% \newcommand {\WHILE}{{\bf while\ }}
% \newcommand {\ACCEPT}{{\bf accept}}
% \newcommand {\REJECT}{\mbox{\bf reject}}
% \newcommand {\THEN}{\mbox{\bf then\ }}
% \newcommand {\END}{{\bf end}}
% \newcommand {\RETURN}{\mbox{\bf return\ }}
% \newcommand {\HALT}{\mbox{\bf halt}}
% \newcommand {\REPEAT}{\mbox{\bf repeat\ }}
% \newcommand {\UNTIL}{\mbox{\bf until\ }}
% \newcommand {\TRUE}{\mbox{\bf true\ }}
% \newcommand {\FALSE}{\mbox{\bf false\ }}
% \newcommand {\FORALL}{\mbox{\bf for all\ }}
% \newcommand {\DOWNTO}{\mbox{\bf down to\ }}

%% %formatting commands
%% \newcounter{lecnum}
%% \newcommand{\lecture}[3]{%
%% \pagestyle{myheadings}%
%% \thispagestyle{plain}%
%% \newpage %
%% \setcounter{lecnum}{#1}%
%% \setcounter{page}{1}%
%% %\rule{\linewidth}{1mm}
%% \begin{center}
%% \shadowbox{\parbox{4.3in}{{\small {\bf {\sc Georgia Tech  Fall'04
%%  \\ \hfill CS 8002 : PCPs and Hardness of Approximation}}}

%% \medskip

%% \begin{center}
%% {\large Lecture #1: #2}
%% \end{center}

%% \medskip

%% Lecturer: {\em Subhash Khot} \hfill Scribe:{\em #3}
%% \vspace{2pt}}}
%% \vspace{6pt}\end{center}}

%% %%%%%%%%    SPRING'01
%% \newcommand{\coursenum}{CS278}
%% \newcommand{\coursename}{Computational Complexity}
%% \newcommand{\courseprof}{Professor Luca Trevisan}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Commands to include figures


%% PSfigure

\newcommand{\PSfigure}[3]{\begin{figure}[t]
  \centerline{\vbox to #2 {\vfil \psfig{figure=#1.eps,height=#2} }}
  \caption{#3}\label{#1}
  \end{figure}}

\newcommand{\twoPSfigures}[5]{\begin{figure*}[t]
  \centerline{%
    \hfil
    \begin{tabular}{c}
        \vbox to #3 {\vfil\psfig{figure=#1.eps,height=#3}} \\ (a)
    \end{tabular}
    \hfil\hfil\hfil
    \begin{tabular}{c}
        \vbox to #3 {\vfil\psfig{figure=#2.eps,height=#3}} \\ (b)
    \end{tabular}
    \hfil}
  \caption{#4}
  \label{#5}
%  \sublabel{#1}{(a)}
%  \sublabel{#2}{(b)}
  \end{figure*}}


\newcounter{fignum}

% fig
%command to insert figure. usage \fig{name}{h}{caption}
%where name.eps is the postscript file and h is the height in inches
%The figure is can be referred to using \ref{name}
\newcommand{\fig}[3]{%
\begin{minipage}{\textwidth}
\centering\epsfig{file=#1.eps,height=#2}
\caption{#3} \label{#1}
\end{minipage}
}%


% ffigure
% Usage: \ffigure{name of file}{height}{caption}{label}
\newcommand{\ffigure}[4]{
\begin{figure}
\caption{#3}
\label{#4}
\centerline{\vbox to #2 {\hfil \psfig{figure=#1.eps,height=#2} }}
\end{figure}
}

% ffigureh
% Usage: \ffigureh{name of file}{height}{caption}{label}
\newcommand{\ffigureh}[4]{
\begin{figure}[!h]
\caption{{\small {\sc #3}}}
\label{#4}
\centerline{\vbox to #2 {\vfil \psfig{figure=#1.eps,height=#2} }}
\end{figure}
}

\newcommand{\pdffigureh}[4]{\begin{figure}[!h]
  \centerline{\vbox to #2 {\vfil \pdffig{figure=#1.eps,height=#2} }}
  \caption{{\small {\sc #3}}}\label{#4}
  \end{figure}}

%beautifications
\def\bsq{\begin{flushright}$\blacksquare$\end{flushright}}
\def\ni{\noindent}


%mystuff


\newcommand{\opt}{\mbox{\rm OPT}}
\newcommand{\alg}{\mbox{\rm ALG}}
\renewcommand{\deg}{\mbox{\rm deg}}
\newcommand{\outdeg}{\mbox{\rm outdeg}}
\newcommand{\ra}{\rightarrow}
\newcommand{\R}{\mbox{\rm\bf R}}
\newcommand{\Rplus}{\R_+}
\newcommand{\minimize}{\mbox{\rm minimize }}
\newcommand{\maximize}{\mbox{\rm maximize }}
\newcommand{\parent}{\mbox{\rm parent }}
\newcommand{\st}{\mbox{\rm subject to }}
\newcommand{\C}{\mbox{${\cal C}$}}
\newcommand{\F}{\mbox{${\cal F}$}}
\newcommand{\li}{\mbox{${\lambda_i}$}}
\renewcommand{\O}{\mbox{${\cal O}$}}
%\renewcommand{\aa}{\mbox{$\alpha$}}
\newcommand{\ah}{\mbox{$\aa_{INC}$}}
%\renewcommand{\bb}{\mbox{\boldmath $\beta$}}
%\newcommand{\bh}{\mbox{$\bb_{INC}$}}
\renewcommand{\tt}{\mbox{\boldmath $t$}}
\newcommand{\rr}{\mbox{\boldmath $r$}}
\newcommand{\at}{\mbox{$\tt_{INC}$}}
\newcommand{\ar}{\mbox{$\rr_{INC}$}}
\newcommand{\aq}{\mbox{$\qq_{INC}$}}
\newcommand{\x}{\mbox{\boldmath $x$}}
\newcommand{\y}{\mbox{\boldmath $y$}}
\newcommand{\z}{\mbox{\boldmath $z$}}
\newcommand{\e}{\mbox{\boldmath $e$}}
\def\p{\mbox{\boldmath $p$}}
\def\q{\mbox{\boldmath $q$}}
%\def\q{{\boldmath q \unboldmath}}
\def\X{{\mbox{\boldmath $X$}}}
\def\x{\mbox{\boldmath $x$}}
\def\e{\mbox{\boldmath $e$}}
\def\U{\mbox{\boldmath $U$}}
\def\a{\mbox{\boldmath $s$}}
\def\s{\mbox{\boldmath $s$}}
\def\m{\mbox{\boldmath $m$}}
\def\b{{\bf b}}
\def\Int{\mbox{\rm Int}}
\def\eps{\epsilon}
\def\uij{u_{ij}}
\def\uijl{u_{ij}^l}
\def\Bijl{B_{ij}^l}
\def\lijk{l_{ij}^k}
\def\g{\mbox{\boldmath $g$}}
\def\f{\mbox{\boldmath $f$}}
\newcommand{\lone}[1]{\ensuremath{|#1|}}
\newcommand{\Real}{\mbox{\rm\bf R}}
\newcommand{\A}{\mbox{\boldmath $\alpha$}}
%\newcommand{\B}{\mbox{\boldmath $\beta$}}
\newcommand{\ga}{\mbox{\boldmath $\gamma$}}
\newcommand{\ltwo}[1]{\|#1\|}
\newcommand{\Cs}{\mbox{{\cal C}}}
%\newcommand{\L}{\mbox{${\cal L}$}}
\newcommand{\Z}{\mbox{\rm\bf Z}}
\newcommand{\Zplus}{\Z^+}
\newcommand{\CA}{\mbox{${\cal A}$}}
\renewcommand{\span}{\mbox{\rm span}}


\newcommand{\pp}{\mbox{\boldmath $p$}}
\newcommand{\mm}{\mbox{\boldmath $m$}}
\renewcommand{\aa}{\mbox{\boldmath $a$}}
\renewcommand{\ss}{\mbox{\boldmath $s$}}
\newcommand{\bp}{\mbox{$\pp_{DEC}$}}
\newcommand{\ap}{\mbox{$\pp_{INC}$}}
\newcommand{\bq}{\mbox{$\qq_{DEC}$}}
\newcommand{\br}{\mbox{$\rr_{DEC}$}}
%\newcommand{\implies}{\mbox{${\Rightarrow}$}}
\newcommand{\eat}[1]{}

\newcommand{\maxi}{{\hbox{\rm maximize}}}
\newcommand{\mini}{{\hbox{\rm minimize}}}
\newcommand{\subjto}{{\hbox{\rm subject to}}}
%\newcommand{\text}[1]{\hbox{\rm #1}}

\def\d{\displaystyle}

\newcommand{\assign}{\leftarrow}


\renewcommand{\u}{\mbox{\boldmath $u$}}
\renewcommand{\v}{\mbox{\boldmath $u$}}
\def\c{{\bf c}}
\renewcommand{\t}{\mbox{\boldmath $t$}}
%\newcommand{\m}{\mbox{\boldmath $m$}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\Pu}{\mathcal{P}_u}
\newcommand{\Pf}{\mathcal{P}_f}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\D}{\mathcal{D}}


\newcommand{\ipj}{\ensuremath{I_{j,j+1}}}
\newcommand{\ipl}{\ensuremath{I_{l,l+1}}}

\newcommand{\aij}{ a_{ij}}
\newcommand{\cij}{ c_{ij}}
\newcommand{\akj}{ a_{kj}}
%\newcommand{\uij}{ u_{ij}}
\newcommand{\xij}{ x_{ij}}
\newcommand{\aijp}{ a_{kj}}
\newcommand{\uis}{\ensuremath{u_1^l}}
\newcommand{\uts}{\ensuremath{u_2^l}}
\newcommand{\ups}{(\uis,\uts)}
\newcommand{\vis}{\ensuremath{v_1^k}}
\newcommand{\vts}{\ensuremath{v_2^k}}
\newcommand{\vps}{(\vis,\vts)}
\newcommand{\lpi}{_{\l+1}}
\renewcommand{\v}{u^{l-1}}
\newcommand{\w}{u^{l}}
\newcommand{\calM}{\mbox{${\cal M}$}}
\newcommand{\CP}{\mbox{${\cal P}$}}
\renewcommand{\Pi}{\mathcal{P}}
%\renewcommand{\Theta}{\mathcal{D}}


\newlength{\lpskip}
\lpskip 4pt

\newcommand{\finv}{f_j^{-i}}
\newcommand{\ginv}{g_j^{-i}}

\newcommand{\cost}{\mbox{\rm cost}}
\newcommand{\seg}{\mbox{\rm seg}}
\newcommand{\segs}{\mbox{\rm segments}}
\newcommand{\valuex}{\mbox{\rm value}}
\newcommand{\rate}{\mbox{\rm rate}}
\newcommand{\spent}{\mbox{\rm spent}}
\newcommand{\all}{\mbox{\rm allocated}}
\newcommand{\allocated}{\mbox{\rm allocated}}
\newcommand{\ret}{\mbox{\rm returned}}
\newcommand{\good}{\mbox{\rm good}}
\newcommand{\best}{\mbox{\rm best}}
\newcommand{\bestT}{\mbox{\rm bestT}}
\newcommand{\fr}{\mbox{\rm fr}}
\newcommand{\fl}{\mbox{\rm fl}}
\newcommand{\bfr}{\mbox{\rm {\bf freeze}}}
\newcommand{\bpb}{\mbox{\rm bpb}}

\newcommand{\bxi}{\mbox{\boldmath $\xi$}}
\newcommand{\bzeta}{\mbox{\boldmath $\zeta$}}
\newcommand{\tS}{\ensuremath{\tilde{S}}}


%project specific
\newcommand{\alfail}{ \alpha_{il}}
\newcommand{\micap}{\hat{m}_i}
\newcommand{\sjcap}{\hat{s}_j}
\newcommand{\xijl}{ x_{ij}^l}
\newcommand{\uil}{ \u_{i}^l}
\newcommand{\lil}{ \lambda_{i}^l}
\newcommand{\muil}{ \mu_{i}^l}
\newcommand{\wil}{ w_{i}^l}
\newcommand{\bij}{ b_{ij}}
\newcommand{\bijl}{ b_{ij}^l}
\newcommand{\fij}{ f_{ij}}
\newcommand{\phij}{ \phi_{ij}}
\newcommand{\sca}{S \subseteq A}
\newcommand{\tcb}{T \subseteq B}
\newcommand{\bphi}{\mbox{\boldmath $\phi$}}
\newcommand{\poly}{\mathcal{P}}
\newcommand{\Lg}{{\mathcal{L}}_{\p}}
\newcommand{\one}{\mathds{1}}



\newcommand{\ipdf}[3]{
\begin{figure}[ht]
\label{#3}
\includegraphics[scale=#1]{#2}
\end{figure}
}











